Fog Function: Serverless Fog Computing for Data Intensive IoT Services

Fog computing can support IoT services with fast response time and low bandwidth usage by moving computation from the cloud to edge devices. However, existing fog computing frameworks have limited flexibility to support dynamic service composition with a data-oriented approach. Function-as-a-Service (FaaS) is a promising programming model for fog computing to enhance flexibility, but the current event- or topic-based design of function triggering and the separation of data management and function execution result in inefficiency for data-intensive IoT services. To achieve both flexibility and efficiency, we propose a data-centric programming model called Fog Function and also introduce its underlying orchestration mechanism that leverages three types of contexts: data context, system context, and usage context. Moreover, we showcase a concrete use case for smart parking where Fog Function allows service developers to easily model their service logic with reduced learning efforts compared to a static service topology. Our performance evaluation results show that the Fog Function can be scaled to hundreds of fog nodes. Fog Function can improve system efficiency by saving 95% of the internal data traffic over cloud function and it can reduce service latency by 30% over edge function.

==> sections/04-orchestration.tex <==

\section{Context-driven Orchestration Framework}


FogFlow is a distributed execution framework that dynamically orchestrates elastic services over cloud and edges, in order to reduce internal bandwidth consumption and offer low latency. The unique feature of FogFlow is context-driven, meaning that FogFlow is able to orchestrate dynamic data processing flows over cloud and edges based on three types of contexts, including:

\subsection{System Design}


\emph{System context}: available resources which are changing over time. The resources in a cloud-edge environment are geo-distributed in nature and they are dynamically changing over time; As compared to cloud computing, resources in such a cloud-edge environment are more heterogeneous and dynamic.

\emph{Data context}: the structure and registered metadata of available data, including both raw sensor data and intermediate data. Based on the standardized and unified data model and communication interface, namely NGSI, FogFlow is able to see the content of all data generated by sensors and data processing tasks in the system, such as data type, attributes, registered metadata, relations, and geo-locations. 

\emph{Usage context}: high level intents defined by all different types of users (developers, service consumers, data providers) to specify what they want to achieve. For example, for service consumers, they can specify which type of results is expected under which type of QoS within which geo-scope; for data providers, they can specify how their data should be utilized and by whom.

\begin{figure}[h]
\centerline{\includegraphics[width=\linewidth]{fig/arch.pdf}}
\caption{System Architecture}
\label{fig:arch}
\end{figure}


\subsection{Content-based Discovery}

Two-layer data management

partial update, availability subscription

design of IoT Discovery to have high throughput

\subsection{Context-driven Orchestration}

Figure 3 shows the major procedure for FogFlow Orchestrator to carry out the advanced task deployment and task migration algorithms, 
based on the update of context available provided by IoT Discovery.  
As been illustrated in the figure, FogFlow Orchestrator is at the top service orchestration layer. 
At the bottom is the device layer, which includes all context producers and consumers (for example, sensors like temperature sensors, cameras, or parking sensors, actuators like connected speakers/displays or connected moving cars; external applications can be contex producers/consumers as well). In between is the cloud-edge computing environment that consists of a large number of FogFlow workers deployed at all edge nodes (e.g., IoT Gateways) and cloud nodes (e.g., Virtual Machines from Google/Amazon Cloud).  In addition, there are also lots of Edge Brokers deployed at edge nodes, managing all context entities and updates from the device layer. More importantly for the service orchestration, the latest context data are indexed by IoT Discovery to provide the updated context availability information required by FogFlow Orchestrator to orchestration IoT services. 
As shown in Figure 3, the major steps are listed as below: 

Step 1: Service designers use the FogFlow dashboard to design the service logic of their IoT Services (namely service template, the detail has been provided in the previous deliverable D4.2 [2]); once the service logic design has been finished, they can submit the services to FogFlow Orchestration to finish the registration of an IoT service;

Step 2: On receiving a registered service template, FogFlow Orchestrator starts to subscribe availability updates of context entities required by the tasks within the service template; 

Step 3: If some new device joins the FogFlow system by connecting to its nearby FogFlow Edge Broker, the entity of this device will be automatically indexed by IoT Discovery to represent the availability of this device. If the context entity type produced by this device is matched with what the registered service template requires, “Notification” will be sent to FogFlow Orchestrator for the purpose of triggering or updating the data processing flows of registered IoT Services. 

Step 4: Once FogFlow Orchestrator receives a notification message of context availability from IoT Discovery, it will start to check if any orchestration action is necessary to be triggered. If necessary, it will generate the required orchestration actions and assign them to the corresponding FogFlow Worker. Currently, four orchestration actions are introduced:  adding a new task instance, removing an existing task instance, adding a new input stream for a running task instance, removing an input stream for a running task instance. More detailed algorithms on how to generate orchestration actions from the notification will be introduced in the following section. 

Step 5: Once a FogFlow Worker receives an orchestration action, it will perform the action accordingly.  What needs to be done for each orchestration action will be described in the following sections. 

Step 6: Each task instance is associated with an operator, which is implemented as a dockerized application. When launching a task instance, the FogFlow Worker needs to fetch the docker image of the corresponding operator from a public/private docker registry. 

Step 7: After the data processing task instances have been launched by FogFlow Workers, various results will be produced and published back to the FogFlow internal context management system. Those results might be forwarded to external context subscribers like an Alarm device. 

The following four basic orchestration actions are designed and implemented in FogFlow for FogFlow Workers to dynamically orchestrate the data processing flows of IoT services in a cloud-edge based environment. 

\emph{ADD\_TASK}: To launch a new task instance with the given configuration that includes the initial setting of its input streams. When launching a new task instance, the FogFlow Worker will first fetch the docker image for this task and then launch and configure this task instance within a dedicated docker container. After that, the FogFlow Worker will subscribe the input entity to the FogFlow context management system on behalf of the running task instance so that the input streams can be received by the running task instance; in the end, the newly created task instance will be reported back to the FogFlow system. 

\emph{REMOVE\_TASK}: To terminate an existing running task instance with the given task ID. When terminating an existing task instance, the FogFlow Worker not only stops and removes its corresponding docker container, but also unsubscribes its input streams so that the FogFlow context management system does not end up with lots of unavailable subscribers. 

\emph{ADD\_INPUT}: To subscribe a new input stream on behalf of a running task instance so that the new input stream can flow into the running task instance. 

\emph{REMOVE\_INPUT}: To unsubscribe some existing input stream on behalf of a running task instance so that the task instance stop receiving entity updates from this input stream. 


\begin{figure}[h]
\centerline{\includegraphics[width=\linewidth]{fig/orchestration.pdf}}
\caption{Context-driven Orchestration}
\label{fig:orchestration}
\end{figure}

\subsection{Algorithms of Task Deployment and Migration}

Task migration is the combined orchestration action of removing an existing task instance on FogFlow Worker A and adding a new task instance on another FogFlow Worker B. Currently, FogFlow can only support the migration of a stateless stream processing task, meaning that the stream processing task does not hold any persistent state and terminating or restarting the task instance does not lead to any faulty result and only affect the parallelism of the task. Depending on where the FogFlow Worker A and B are located in the cloud-edge environment, FogFlow can allow seamless task migration from the cloud to an edge, from an edge to the cloud, or from one edge to another edge. Here we list some typical scenario examples to when various task migration procedures are expected to happen. 

\emph{Cloud $->$ Edge}: for example, if a new edge node joins the FogFlow system and it is close to one edge device, a task instance running in the cloud can be migrated from the central cloud to this new edge node in order to save bandwidth cost. 

\emph{Edge $->$ Cloud}: for example, when an edge node becomes overloaded when it has to handle the workload from lots of devices in the same region, it can start to migrate some existing task instances to the cloud in order to keep enough resource for the other urgent task instances. 

\emph{Edge $->$ Edge}: for example, when a mobile device like a connected car or flying drone moves from one region (R1) to another region (R2), it might find another nearby edge node that can provide lower latency. In this case, it is better to migration the task instance to the edge node in R2. In this case, task instances are migrated in order to adapt to the mobility of connected devices. 

algorithms of task assignment


adaptive to the changing workload


